Super-Resolution with Deep Adaptive Image Resampling

Deep learning based methods have recently pushed the state-of-the-art on the problem of Single Image Super-Resolution (SISR). In this work, we revisit the more traditional interpolation-based methods, that were popular before, now with the help of deep learning. In particular, we propose to use a Convolutional Neural Network (CNN) to estimate spatially variant interpolation kernels and apply the estimated kernels adaptively to each position in the image. The whole model is trained in an end-to-end manner. We explore two ways to improve the results for the case of large upscaling factors, and propose a recursive extension of our basic model. This achieves results that are on par with state-of-the-art methods. We visualize the estimated adaptive interpolation kernels to gain more insight on the effectiveness of the proposed method. We also extend the method to the task of joint image filtering and again achieve state-of-the-art performance.

==> intro_long.tex <==
% sampling based methods (bilinear, bicubic, lanczos)
% sparse coding/dictionary based methods
% deep learning based methods 
% (directly conv to generate super-res result from scratch like srcnn or espcnn;
% use cnn to compute residual and combined with precomputed bicubic interpolation result as result)

Reconstructing a high-resolution (HR) image from a low-resolution (LR) input is a classic computer vision problem, referred as {\em Single Image Super-Resolution} (SISR). Research on SISR receives a lot of attention because of the wide range of applications, such as surveillance, medical imaging and remote sensing imaging, where high-frequency details are required. 
The main difficulty with SISR lies in the fact that it is an ill-posed problem: the high-frequency information is missing and there are many possible solutions that are consistent with the given low-resolution input. Therefore, additional assumptions have to be made regarding the formation of HR images. A common key assumption for this task is that the high-frequency information is redundant and can be reconstructed either from the given LR image or from external exemplars.

% theory motivated methods, interpolation/filtering
Basic methods for SISR are general {\em interpolation based methods}, such as bilinear interpolation, bicubic interpolation and Lanczos resampling~\cite{Blu-tip04}. These methods are motivated either by the sampling theorem or spline theory [Splines - A perfect fit for signal and image processing]. In Nyquist-Shannon sampling theory, the optimal reconstruction filter for band-limited continuous signals is the sinc filter and the reconstruction is a linear combination of sinc functions. 
%However, the sinc interpolation kernel is impossible to implement since it has infinite support. Therefore, 
In practice, people use Lanczos resampling as a finite-length approximation of the infinite sinc function.
These traditional interpolation methods assume a band-limited continuous signal and apply a fixed interpolation kernel to the LR image to achieve the upscaling. As a result, they cannot adapt to the content of the image, often resulting in aliasing artifacts or over-smoothed regions. 
%
To address this issue, several works~\cite{Zhang-tip06,Takeda-tip07,Zhou-ietip12} have proposed {\em edge guided image interpolation methods}. They use prior information about the images as regularization such that they are able to upscale the image while keeping the edges sharp. In a similar spirit, He~\etal~\cite{He-tpami13} proposed a guided image filter where spatially variant filters are computed for an edge-preserving smoothing operation. This is applied to several image editing tasks, including SISR.

% learning based / data-driven based methods
Recent methods which work well on SISR learn a mapping between LR space and HR space in a data-driven fashion. One family of methods falling in this category are {\em dictionary based methods}~\cite{Chang-cvpr04, Yang-cvpr08, Timofte-iccv13, Timofte-accv14}. They explicitly learn a dictionary mapping between LR space and HR space. Once the mapping is learned, the same set of coding coefficients computed for the LR image are used for the HR image to produce the super-resolved result. 
Another family of data-driven methods are {\em deep learning based models}~\cite{Dong-tpami16, Dong-eccv16, Shi-cvpr16}. Building on the powerful capability of deep neural networks, these methods learn an implicit mapping between LR and HR images with a fully-convolutional network in an end-to-end manner. Deeper networks~\cite{Kim-cvpr16-vdsr, Kim-cvpr16-drcn, Mao-nips16,Caballero-cvpr17} have been proposed to further improve the performance and currrently define the state-of-the-art.

\begin{figure*}[t]
    \begin{tabular}{cc}
    	\begin{adjustbox}{valign=c}
			\begin{tabular}{c}
				\includegraphics[width=0.45\linewidth]{./images/pipeline_SRCNN.pdf}
				\\[1ex]
				(a) SRCNN~\cite{Dong-tpami16}
				\\[1ex]
				\includegraphics[width=0.45\linewidth]{./images/pipeline_VDSR.pdf}
				\\[1ex]
				(b) VDSR~\cite{Kim-cvpr16-vdsr}
				\end{tabular}
		\end{adjustbox}
		&
        \begin{adjustbox}{valign=c}
			\begin{tabular}{c}
				\includegraphics[width=0.45\textwidth]{./images/pipeline.pdf}
				\\[1ex]
				(c) Ours
			\end{tabular}
		\end{adjustbox}
    \end{tabular}	
    \caption{Network architecture comparison between our method and SRCNN and VDSR.}
    \label{fig:pipeline}
\end{figure*} 
% Though the above deep learning based models obtain very good super-resolution result, it is not that obvious to know what the NN has learned.
In this work, instead of further increasing the network depth, we revisit the idea of interpolation based methods, but now with the help of deep learning, aiming at an effective model with some insights. Similar in spirit to the edge guided image interpolation~\cite{He-tpami13}, we compute a pixel in a high-resolution image using interpolation, \ie using a weighted average of the nearby pixels in the corresponding low-resolution image, where the weights are not fixed but depend on the image content at that position. Therefore, the interpolation kernels are spatially variant and content-aware. For example, in smooth regions, there is not much variance among pixels in a neighborhood, so a uniform kernel might do a reasonable job; however, for regions corresponding to edges, kernels dominated by only one or a few non-zero elements, might produce sharper edges; for a region with rich texture, a specially-designed combination of neighboring pixels is required for its interpolation. 

Instead of using hand-designed kernels to do the filtering/interpolation, we propose to use a deep neural network to learn good interpolation kernels in a data-driven fashion. For this, we build on the recently proposed Dynamic Filter Network architecture of~\cite{DeBrabandere-nips16}.

Deep neural networks are known for their powerful modeling capability. They are able to learn a more advanced mapping function for input and output pairs than methods like the guided image filter, which uses a local linear model~\cite{He-tpami13}. For example, deep neural networks are able to recognize not only the pattern of a region (smooth region/edge/textured region) but also its semantic meaning, which may help in figuring out a suitable way to combine its nearby pixels for its super-resolving. 

Once the adaptive interpolation kernels are estimated, we add an interpolation/resampling layer
which carries out the actual filtering operation
(see Figure~\ref{fig:pipeline}c): the estimated interpolation kernels are applied to a low resolution image to obtain the super-resolved result. The proposed interpolation/resampling layer is similar to the bilinear upsampling layer proposed in~\cite{Jaderberg-nips15}. The added module is differentiable and allows end-to-end training for the whole model. However, in our case the weights are computed by the network and the size of the kernel can be designated as a hyperparameter. 

The performance of interpolation-based methods drops as the upscaling factor increases. That is because when the upscaling factor is big, there is little correlation among nearby pixels. In this case non-local methods perform better than local linear filtering methods. We explore two ways to address the degeneration in case of large upscaling factor for interpolation-based methods: an atrous spatial pyramid and progressive upsampling. Besides, the deep adaptive image resampling can be applied to the previously obtained super-resolution result several times, i.e. in a recurrent fashion, to further improve the performance.
%
% (\xu{To focus more on a novel point of view to address the super-res problem. Should I change the term to adaptive image resampling/interpolation network and use it to replace the dynamic filter network one (and I will only mention dfn in related work?})
% Recently~\cite{Finn-nips16,DeBrabandere-nips16,Xue-nips16} simultaneously proposed a model (called Dynamic Filter Networks (DFN) in~\cite{DeBrabandere-nips16} and will also be used in this paper) that is able to generate adaptive spatial transformation to address video prediction task. An input is fed to a filter generation network to produce sample-specific and position-specific filters which model spatial transformations at each position and the next frame is predicted by applying those filters to one previous frame at different positions. Inspired by this idea, we propose to compute content-aware interpolation kernels for different images and positions to adapt to various textures and patterns. Image resampling is then done with one single filtering step. 
% (\xu{too many implementation details})
% Kernels are computed with a filter generation network and applied to each position in LR image to produce the interpolated super-resolution result. Since LR image and HR image have different sizes, we need to make two modifications compared to the original DFN. First, the filter generation network is required to generate more than one filters for each position in the input LR space according to the requirement of upscaling. Therefore, an upsampling layer is added to the end of filter generation network. Second, LR image is resized to the same size of HR image using nearest neighbor method before sent to dynamic filtering layer. The dynamic filtering operation is extended to allow filtering with various sampling rate, similar to dilated convolution, such that different filters are applied to the same set of neighboring pixels in the original LR space for interpolation. 
%
% (\xu{aspp, recursive model, vdsr+dfn, joint filtering with guidance})

The proposed methods are evaluated on four super-resolution benchmark datasets and perform favorably compared to state-of-the-art methods.
% in both accuracy, speed and memory.
We visualize the estimated interpolation kernels and shed some light on why the proposed method works well.
%
In addition, we show that the proposed method can be naturally extended for the joint image filtering task and again obtains state-of-the-art performance.

% Contributions:
% a new way to address image super-resolution task with deep learning model;
% analyze what is learned with the deep learning model;
% joint image filtering;
